Taking out the Toxic Trash: Recovering Precision in Mixed Flow-Sensitive Static Analyses

Static analysis of real-world programs combines flow- and context-sensitive analyses of local program states with computation of flow- and context-insensitive invariants at globals, that, e.g., abstract data shared by multiple threads. The values of locals and globals may mutually depend on each other, with the analysis of local program states both making contributions to globals and querying their values. Usually, all contributions to globals are accumulated during fixpoint iteration, with widening applied to enforce termination. Such flow-insensitive information often becomes unnecessarily imprecise and can include superfluous contributions -- trash -- which, in turn, may be toxic to the precision of the overall analysis. To recover precision of globals, we propose techniques complementing each other: Narrowing on globals differentiates contributions by origin; reluctant widening limits the amount of widening applied at globals; and finally, abstract garbage collection undoes contributions to globals and propagates their withdrawal. The experimental evaluation shows that these techniques increase the precision of mixed flow-sensitive analyses at a reasonable cost.

==> Makefile <==
all:
	pdflatex main.tex
	bibtex main.aux
	pdflatex main.tex
	pdflatex main.tex

fast:
	pdflatex main.tex
	bibtex main.aux

grayscale:
	pdflatex -jobname grayscale '\PassOptionsToPackage{gray}{xcolor}\input main.tex'
	bibtex grayscale.aux
	pdflatex -jobname grayscale '\PassOptionsToPackage{gray}{xcolor}\input main.tex'
	pdflatex -jobname grayscale '\PassOptionsToPackage{gray}{xcolor}\input main.tex'

clean:
	rm *.blg *.bbl *.aux *.log


==> data/reachsafety-recursive-context0/timeout-counts.tex <==
\newcommand\casecountrec{156}
\newcommand\incompleterec{0}
\newcommand\incompleterecoursth{0}
\newcommand\incompleterecourstwz{0}
\newcommand\incompleterecbase{0}
\newcommand\incompleterecapinis{0}


==> sections/update_rules/always_widen.tex <==
\begin{figure}
    \begin{lstlisting}[style=ccode,caption={\label{lst:always_widen}Update rule for globals to handle contributions triggered by right-hand sides by always joining.}]
update_globals($\Locals$ orig, $2^{\Globals\times\Dom}$ contribs, $\Globals\to\Dom$ $\rho$) {
  updates = $\emptyset$; // Updates to be propagated to the solver
  foreach((g,b) $\in$ contribs) { // Iterate over contributions
    if(b $\sqsubseteq$ $\rho$ g) continue; // Nothing to do
    updates = updates $\cup$ {(g,$\rho$ g $\widen b$)}; // Compute new value by widening
  }
  return updates;
}
    \end{lstlisting}
\end{figure}

